GraphTranslator: Aligning Graph Model to Large Language Model for Open-ended Tasks

Large language models (LLMs) like ChatGPT, exhibit powerful zero-shot and instruction-following capabilities, have catalyzed a revolutionary transformation across diverse fields, especially for open-ended tasks. While the idea is less explored in the graph domain, despite the availability of numerous powerful graph models (GMs), they are restricted to tasks in a pre-defined form. Although several methods applying LLMs to graphs have been proposed, they fail to simultaneously handle the pre-defined and open-ended tasks, with LLM as a node feature enhancer or as a standalone predictor. To break this dilemma, we propose to bridge the pretrained GM and LLM by a Translator, named GraphTranslator, aiming to leverage GM to handle the pre-defined tasks effectively and utilize the extended interface of LLMs to offer various open-ended tasks for GM. To train such Translator, we propose a Producer capable of constructing the graph-text alignment data along node information, neighbor information and model information. By translating node representation into tokens, GraphTranslator empowers an LLM to make predictions based on language instructions, providing a unified perspective for both pre-defined and open-ended tasks. Extensive results demonstrate the effectiveness of our proposed GraphTranslator on zero-shot node classification. The graph question answering experiments reveal our GraphTranslator potential across a broad spectrum of open-ended tasks through language instructions. Our code is available at: https://github.com/alibaba/GraphTranslator.

==> alt-text.tex <==
Figure 1: \Description[Our minimum-budget attack can is better than fixed-budget attack.]{Existing fixed-budget topology attacks may fail to cross decision boundary or cross too much. While our MiBTack can exactly cross the closest green decision boundary with no waste.}

Figure 2: \Description[The framework of our MiBTack.]{ The overall procedure of our proposed MiBTack in $i$-th iteration.}

Figure 3: \Description[The node classification margins under our MiBTack.]{Compared to other attacks, our MiBTack leads all target nodes misclassified and affects them most slightly in the meantime.}

Figure 4: \Description[Our MiBTack can handle poisoning attack setting.]{Our MiBTack lead most target nodes misclassified even under poisoning attack setting.}

Figure 5: \Description[Our MiBTack can achieve better attack performance against defensed GNNs.]{Even GCN is defensed (JacGCN and RGCN), our variants MiBTack-J and MiBTack-R can achieve better attacks compared with Nettack.}

Figure 6: \Description[Impact of patience $P$ on MiBTack.]{MiBTack obtains lower minimum budget with the increasing of patience $P$ and only requires a few of the trials to converge.}

Figure 7: \Description[Impact of step size $\alpha$ on MiBTack.]{There exists an optimal $\alpha$ that delivers the minimum budget.}

Figure 8: \Description[Impact of step size $\beta$ on MiBTack.]{The performance of MiBTack is stable when $\beta$ is within the range from $\{0.005, 0.01, 0.05, 0.1, 0.5, 1\}$.}

Figure 9: \Description[Relationships of node robustness and degree.]{There is a positive correlation between degree and node robustness.}


Figure 10: \Description[Relationships of node robustness and uncertainty.]{There may exist a turning point for GNNs from over-confident to under-confident.}

